COARA: Code Offloading on Android with AspectJ

Smartphones suffer from limited computational capabilities and battery life. A method to mitigate these problems is code offloading: executing application code on a remote server. We introduce COARA, a middleware platform for code offloading on Android that uses aspect-oriented programming (AOP) with AspectJ. AOP allows COARA to intercept code for offloading without a customized compiler or modification of the operating system. COARA requires minimal changes to application source code, and does not require the application developer to be aware of AOP. Since state transfer to the server is often a bottleneck that hinders performance, COARA uses AOP to intercept the transmission of large objects from the client and replaces them with object proxies. The server can begin execution of the offloaded application code, regardless of whether all required objects been transferred to the server. We run COARA with Android applications from the Google Play store on a Nexus 4 running unmodified Android 4.3 to prove that our platform improves performance and reduces energy consumption. Our approach yields speedups of 24x and 6x over WiFi and 3G respectively.

==> FinalDataPerformance2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Chess Speedup	&WiFi	&3G\\
Overall	&4.0x	&3.3x\\
Computation only	&9.8x	&6.0x\\
	&	&\\
	&	&\\
	&	&\\
	&	&\\
	&	&\\
\# of Iterations	&WiFi	&3G\\
10	&0.8x	&0.3x\\
15	&1.1x	&0.5x\\
20	&1.7x	&0.8x\\
30	&2.0x	&1.0x\\
40	&2.8x	&1.2x\\
100	&6.4x	&2.6x\\
200	&10.1x	&5.2x\\
500	&10.7x	&10.9x\\
1000	&15.8x	&13.3x\\
	&	&\\
	&	&\\
FD Speedup Image	&WiFi	&3G\\
Eager	&8.1x	&3.3x\\
Lazy	&7.3x	&3.1x\\
Pipelined	&6.4x	&3.5x\\
Cache	&16.6x	&9.6x\\
	&	&\\
FD Speedup Image	&WiFi	&3G\\
Eager	&15.3x	&5.3x\\
Lazy	&10.8x	&4.0x\\
Pipelined	&18.8x	&6.1x\\
Cache	&27.7x	&18.7x\\
	&	&\\
s	&WiFi	&3G\\
Eager	&17.5x	&4.8x\\
Lazy	&11.1x	&3.7x\\
Pipelined	&24.7x	&6.1x\\
Cache	&31.9x	&23.3x\\
	&	&\\
FD Speedup Image	&WiFi	&3G\\
Eager	&2.0x	&0.5x\\
Lazy	&7.6x	&3.1x\\
Pipelined	&3.4x	&0.7x\\
	&	&\\
	&	&\\
	&	&\\
	&	&\\
Benchmark	&6.4	&4.7\\
Chess (30 move game)	&83.5	&75.6\\
FD 1 Image Eager	&196.7	&51.5\\
FD 1 Image Lazy	&196.7	&51.4\\
FD 1 Image Pipelined	&196.3	&50.7\\
FD 1 Image Cache	&1.3	&2.7\\
FD 5 Images Eager	&748.1	&170\\
FD 5 Images Lazy	&748.3	&173\\
FD 5 Images Pipelined	&749.3	&168.1\\
FD 5 Images Cache	&1.6	&7.1\\
FD 10 Images Eager	&1486.9	&327.8\\
FD 10 Images Lazy	&1493.6	&337.3\\
FD 10 Images Pipelined	&1495.6	&327.7\\
FD 10 Images Cache	&1.8	&7.8\\
FD 1/10 Eager	&1487.5	&323.3\\
FD 1/10 Lazy	&117	&28.6\\
FD 1/10 Pipelined	&1494.6	&62.1\\

